The complete one-loop dilatation operator of planar real beta-deformed N=4 SYM theory

We determine the missing finite-size corrections to the asymptotic one-loop dilatation operator of the real $\beta$-deformed $\mathcal{N}=4$ SYM theory for the gauge groups $U(N)$ and $SU(N)$ in the 't Hooft limit. In the $SU(N)$ case, the absence of the $U(1)$ field components leads to a new kind of finite-size effect, which we call prewrapping. We classify which states are potentially affected by prewrapping at generic loop orders and comment on the necessity to include it into the integrability-based description. As a further result, we identify classes of $n$-point correlation functions which at all loop orders in the planar theory are given by the values of their undeformed counterparts. Finally, we determine the superconformal multiplet structure and one-loop anomalous dimensions of all single-trace states with classical scaling dimension $\Delta_0 \leq 4.5$.

==> Macros/DiagramMacro.tex <==
\newcommand{\feynmpdefinitionsdiags}{

\fmfcmd{%
thin := 1pt; % dimension of the lines
thick := 2thin;
arrow_len := 4mm;
arrow_ang := 15;
curly_len := 3mm;
dash_len := 1.8mm; % 'photon' lines
% dash_space := 4mm;
dot_len := 1.5mm; % 'photon' lines
wiggly_len := 2mm; % 'photon' lines
wiggly_slope := 60;
zigzag_len := 2mm;
zigzag_width := 2thick;
decor_size := 5mm;
dot_size := 2thick;
}

\fmfcmd{%
style_def plain_sarrow expr p =
  cdraw p;
  shrink (0.55); %  shrink (0.6);
  cfill (arrow p);
  endshrink;
enddef;
style_def dashes_sarrow expr p =
  draw_dashes p;
  shrink (0.55);
  cfill (arrow p);
  endshrink;
enddef;
style_def plain_srarrow expr p =
  cdraw p;
  shrink (0.55);
  cfill (arrow (reverse p));
  endshrink;
enddef;
style_def dashes_srarrow expr p =
  draw_dashes p;
  shrink (0.55);
  cfill (arrow (reverse p));
  endshrink;
enddef;
%
marksize=2mm;
def draw_mark(expr p,a) =
  begingroup
    save t,tip,dma,dmb; pair tip,dma,dmb;
    t=arctime a of p;
    tip =marksize*unitvector direction t of p;
    dma =marksize*unitvector direction t of p rotated -45;
    dmb =marksize*unitvector direction t of p rotated 45;
    linejoin:=beveled;
    draw (-.5dma.. .5tip-- -.5dmb) shifted point t of p;
  endgroup
enddef;
%
style_def derplain expr p =
    save amid;
    amid=.5*arclength p;
    draw_mark(p, amid);
    draw p;
enddef;
}
}

\newcommand{\nvml}[3][1]{%
%begingroup;
\fmfcmd{%
begingroup;
save a, vp, tvp, nvp, tv, nv, ip, ts, tt, is, it, n, m, scale, t, r, s, ttpr, tnpr, ep, mm;
path lcirc;
pair vp[][], tvp[][], tv[][], nvp[][], nv[][], ip[][], ts[], is[], tt[], it[], ep[], mid;
% number of path segments
n := #2;
% number of points along path segment
m:=3;
for i=1 upto n:
for j=1 upto m:
a[i][j] := arctime ((j-1)/(m-1)*arclength pm[i]) of pm[i];
vp[i][j] := point a[i][j] of pm[i];
tvp[i][j] := unitvector direction a[i][j] of pm[i];
nvp[i][j] := tvp[i][j] rotated -90;
endfor;
endfor;
% decision if path is closed or open
if(vp[1][1]=vp[n][m]):
% closed path
vp[n+1][1] := vp[1][1];
tvp[0][m] := tvp[n][m];
nvp[0][m] := nvp[n][m];
tvp[n+1][1] :=tvp[1][1];
nvp[n+1][1] :=nvp[1][1];
else:
% open path
vp[n+1][1] := vp[n][m];
tvp[0][m] := (0,0);
nvp[0][m] := (0,0);
tvp[n+1][1] :=tvp[n][m];
nvp[n+1][1] :=nvp[n][m];
fi;
% initialization of number of points in the momentum path
s := 1;
for i=1 upto n:
for j=1 upto m:
% tangent and normal vectors at corners (j=1,m)
if (j=1):
tv[i][1] := (tvp[i-1][m]+tvp[i][1]);
nv[i][1] := (nvp[i-1][m]+nvp[i][1]);
if (not(tv[i][1]=(0,0))):
tv[i][1] := unitvector tv[i][1];
fi;
if (not(nv[i][1]=(0,0))):
nv[i][1] := unitvector nv[i][1];
fi;
% inner products of tangent tangent and tangent normal vectors at corners j=1
ttpr := tvp[i][1] dotprod tvp[i-1][m];
tnpr := tvp[i][1] dotprod nvp[i-1][m];
elseif (j=m):
tv[i][m] := (tvp[i][m]+tvp[i+1][1]);
nv[i][m] := (nvp[i][m]+nvp[i+1][1]);
if (not(tv[i][m]=(0,0))):
tv[i][m] := unitvector tv[i][m];
fi;
if (not(nv[i][m]=(0,0))):
nv[i][m] := unitvector nv[i][m];
fi;
ttpr := tvp[i][m] dotprod tvp[i+1][1];
tnpr := -tvp[i][m] dotprod nvp[i+1][1];
else:
nv[i][j] :=nvp[i][j];
tv[i][j] :=tvp[i][j];
fi;
%if(tvp[i-1][m]=tvp[i][1]):
scale := 25;
%else:
%scale := 150/(sqrt(abs(tvp[i-1][m]-tvp[i][1])));
%fi;
if ((j=1) or (j=m)):
 if ((tnpr<=0) and not((tv[i][j]=(0,0)) or (nv[i][j]=(0,0)))):
  ip[i][j] := vp[i][j] shifted(0.15*scale*nvp[i][j]);
  ts[s] := tvp[i][j];
  is[s] := ip[i][j];
  s:=s+1;
 else:
  if ((j=1) and (ttpr>0)):
%   ip[i][j] := vp[i][j] shifted(0.15*scale*nv[i][j]);
%   ts[s] := tv[i][j];
%   is[s] := ip[i][j];
%   s:=s+1;
  fi;
 fi;
else:
 ip[i][j] := vp[i][j] shifted(0.15*scale*nv[i][j]);
 ts[s] := tv[i][j];
 is[s] := ip[i][j];
 s:=s+1;
fi;
endfor;
endfor;
if(vp[1][1]=vp[n][m]):
% closed path
ts[s] := ts[1];
is[s] := is[1];
else:
% open path
tv[n+1][1] := unitvector (tvp[n][m]+tvp[n+1][1]);
nv[n+1][1] := unitvector (nvp[n][m]+nvp[n+1][1]);
ip[n+1][1] := vp[n+1][1] shifted(0.15*scale*nv[n+1][1]);
ts[s] := tv[n+1][1];
is[s] := ip[n+1][1];
fi;
% tension of the momentum loop
t=#1;
lcirc:=is[1];
%draw(is[1]) withpen pencircle scaled 2;
for k=2 upto s:
lcirc := lcirc{ts[k-1]}..tension t..{ts[k]}is[k];
%lcirc := lcirc{ts[k-1]}...{ts[k]}is[k];
%draw(is[k]) withpen pencircle scaled 2;
endfor;
mm := arctime (0.5* arclength lcirc) of lcirc;
if(vp[1][1]=vp[n][m]):
% closed path
ep1 := point arctime (0* arclength lcirc) of lcirc of lcirc;
ep2 := point mm of lcirc;
mid := 1/2[ep1,ep2];
else:
% open path
ep1 := point mm of lcirc;
ep2 :=unitvector direction mm of lcirc rotated -90;
mid:= ep1 shifted(0.2*scale*ep2);
fi;
%lcirc:=is[1]..tension t..{ts[2]}is[2];
%%lcirc:=is[1]...{ts[2]}is[2];
%for k=3 upto (m-1)*n+1:
%if (floor((k-1)/(m-1))=(k-1)/(m-1)):
%lcirc := lcirc{ts[k-1]}..tension t..is[k];
%%lcirc := lcirc{ts[k-1]}...is[k];
%elseif (floor((k-2)/(m-1))=(k-2)/(m-1)):
%lcirc := lcirc..tension t..{ts[k]}is[k];
%%lcirc := lcirc...{ts[k]}is[k];
%else:
%lcirc := lcirc{ts[k-1]}..tension t..{ts[k]}is[k];
%lcirc := lcirc{ts[k-1]}...{ts[k]}is[k];
%fi;
%endfor;
%lcirc:=it[1]{tt[1]}..tension t..{tt[2]}it[2];
%lcirc:=it[1]{tt[1]}...{tt[2]}it[2];
%for k=2 upto (m-2)*n-1:
%lcirc := lcirc;
%lcirc := lcirc{tt[k]}..tension t..{tt[k+1]}it[k+1];
%lcirc := lcirc{tt[k]}...{tt[k+1]}it[k+1];
%endfor;
%lcirc:=lcirc..tension t..{tt[1]}it[1];
draw(lcirc) withpen pencircle scaled 0.25;
drawarrow(subpath(mm*0.8,mm*1.1) of lcirc) withpen pencircle scaled 0.25;
endgroup;
}
\fmfiv{label=#3,l.dist=0}{mid}
}

\newcommand{\svertex}[2]{%
\fmfiequ{#1}{point length(#2)/2 of (#2)}
}
\newcommand{\dvertex}[3]{%
\fmfiequ{#1}{point length(#3)/3 of (#3)}
\fmfiequ{#2}{point 2length(#3)/3 of (#3)}
}
\newcommand{\vvertex}[3]{%
\fmfipath{px}
\fmfiequ{px}{(0,ypart(#2))..(100,ypart(#2))}
\fmfiequ{#1}{point xpart(#3 intersectiontimes px) of (#3)}
%\fmfiequ{ypart(#1)}{ypart(#2)}
}


\newcommand{\aswfone}[4][]{%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-7.5\unitlength}%
%\smash[b]{%
\raisebox{\eqoff}{%
\fmfframe(1,0)(1,0){%
\begin{fmfchar*}(20,15)
\fmfleft{v1}
\fmfright{v2}
\fmffixed{(0.50w,0)}{vc1,vc2}
\fmf{#2}{v1,vc1}
\fmf{#2}{vc2,v2}
\fmf{#3}{vc1,vc2}
\fmf{#4}{vc2,vc1}
\fmffreeze
\fmfposition
\fmfipath{p[]}
\fmfipair{vm[]}
\fmfiset{p1}{vpath(__v1,__vc1)}
\fmfiset{p2}{vpath(__vc1,__vc2)}
\fmfiset{p3}{reverse vpath(__vc2,__vc1) }
\fmfiset{p4}{vpath(__vc2,__v2)}
% \svertex{vm1}{p2}
% \svertex{vm2}{p3}
{#1}
\end{fmfchar*}}}}%}

\newcommand{\aswfonelabel}[6][]{%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-7.5\unitlength}%
%\smash[b]{%
\raisebox{\eqoff}{%
\fmfframe(4,0)(4,0){%
\begin{fmfchar*}(20,15)
\fmfleft{v1}
\fmfright{v2}
\fmffixed{(0.50w,0)}{vc1,vc2}
\fmf{#2}{v1,vc1}
\fmf{#2}{vc2,v2}
\fmf{#3}{vc1,vc2}
\fmf{#4}{vc2,vc1}
%%% Workaround for MetaPost 1.504 bug 
\fmfcmd{pair verta, vertb; verta = vloc(__v1); vertb = vloc(__v2);}
\fmfiv{label=#5,l.a=180,l.dist=0.07w}{verta}
\fmfiv{label=#6,l.a=0,l.dist=0.07w}{vertb}
\fmffreeze
\fmfposition
\fmfipath{p[]}
\fmfipair{vm[]}
\fmfiset{p1}{vpath(__v1,__vc1)}
\fmfiset{p2}{vpath(__vc1,__vc2)}
\fmfiset{p3}{reverse vpath(__vc2,__vc1) }
\fmfiset{p4}{vpath(__vc2,__v2)}
% \svertex{vm1}{p2}
% \svertex{vm2}{p3}
{#1}
\end{fmfchar*}}}}%}

\newcommand{\aswfonelabelf}[6][]{%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-7.5\unitlength}%
%\smash[b]{%
\raisebox{\eqoff}{%
\fmfframe(5,0)(5,0){%
\begin{fmfchar*}(20,15)
\fmfleft{v1}
\fmfright{v2}
\fmffixed{(0.50w,0)}{vc1,vc2}
\fmf{#2}{v1,vc1}
\fmf{#2}{vc2,v2}
\fmf{#3}{vc1,vc2}
\fmf{#4}{vc2,vc1}
%%% Workaround for MetaPost 1.504 bug 
\fmfcmd{pair verta, vertb; verta = vloc(__v1); vertb = vloc(__v2);}
\fmfiv{label=#5,l.a=180,l.dist=0.04w}{verta}
\fmfiv{label=#6,l.a=0,l.dist=0.04w}{vertb}
\fmffreeze
\fmfposition
\fmfipath{p[]}
\fmfipair{vm[]}
\fmfiset{p1}{vpath(__v1,__vc1)}
\fmfiset{p2}{vpath(__vc1,__vc2)}
\fmfiset{p3}{reverse vpath(__vc2,__vc1) }
\fmfiset{p4}{vpath(__vc2,__v2)}
% \svertex{vm1}{p2}
% \svertex{vm2}{p3}
{#1}
\end{fmfchar*}}}}%}


\newcommand{\vacpolp}[2][0.5]{%
\fmfcmd{
begingroup;
save t,v,tv,do,di,ppol,pstr,dia;
path ppol,pstr;
pair v[],tv[],do[],di[];
ppol=#2;
t3=arctime (0.5*arclength ppol) of ppol;
v3=point t3 of ppol;
dia=#1 arclength ppol; 
fill(fullcircle scaled dia shifted v3) withcolor 0.2black;
endgroup;
}
}

\newcommand{\diaglts}[9]{%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-7.5\unitlength}%
%\smash[b]{%
\raisebox{\eqoff}{%
\fmfframe(0,0)(4,0){%
\begin{fmfchar*}(20,15)
\fmfleft{v1}
\fmfright{v0,v2,v5,v6,v7,v3,v4}
\fmf{#1,left=1,tension=0.6}{v1,vc1}
\fmf{#2,right=1,tension=0.6}{v1,vc1}
\fmf{#3,tension=1.5}{vc1,vc2}
\fmf{#4}{vc2,v2}
\fmf{#5}{vc2,v3}
\fmffreeze
\fmfposition
\fmfipath{p[]}
\fmfipair{vm[]}
\fmfiset{p1}{vpath(__v1,__vc1)}
\fmfiset{p2}{vpath(__vc1,__vc2)}
\fmfiset{p3}{reverse vpath(__vc2,__vc1) }
\fmfiset{p4}{vpath(__vc2,__v2)}
% \svertex{vm1}{p2}
% \svertex{vm2}{p3}
%%% Workaround for MetaPost 1.504 bug 
\fmfcmd{pair verta, vertb, vertc; verta = vloc(__v1); vertb = vloc(__v3); vertc = vloc(__v2);}
\fmfiv{label=#6,l.a=110,l.dist=0.27w}{verta}
\fmfiv{label=#7,l.a=-110,l.dist=0.27w}{verta}
\fmfiv{label=#8,l.a=60,l.dist=0.01w}{vertb}
\fmfiv{label=#9,l.a=-60,l.dist=0.01w}{vertc}
%%% Workaround for MetaPost 1.504 bug 
\fmfcmd{pair fubara; fubara = vloc(__v1);} 
\fmfiv{decor.shape=circle,decor.filled=full,decor.size=3}{fubara}
\end{fmfchar*}}}}%}

\newcommand{\diagltt}[9]{%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-7.5\unitlength}%
%\smash[b]{%
\raisebox{\eqoff}{%
\fmfframe(0,0)(4,0){%
\begin{fmfchar*}(20,15)
\fmfleft{v1}
\fmfright{v0,v2,v5,v6,v7,v3,v4}
\fmf{#1,right=0.2,tension=0.6}{v1,vc1}
\fmf{#2,left=0.2,tension=0.6}{v1,vc2}
\fmf{#3,tension=0.1}{vc1,vc2}
\fmf{#4}{vc1,v2}
\fmf{#5}{vc2,v3}
\fmffreeze
\fmfposition
\fmfipath{p[]}
\fmfipair{vm[]}
\fmfiset{p1}{vpath(__v1,__vc1)}
\fmfiset{p2}{vpath(__vc1,__vc2)}
\fmfiset{p3}{reverse vpath(__vc2,__vc1) }
\fmfiset{p4}{vpath(__vc2,__v2)}
% \svertex{vm1}{p2}
% \svertex{vm2}{p3}
%%% Workaround for MetaPost 1.504 bug 
\fmfcmd{pair verta, vertb, vertc; verta = vloc(__v1); vertb = vloc(__v3); vertc = vloc(__v2);}
\fmfiv{label=#6,l.a=110,l.dist=0.27w}{verta}
\fmfiv{label=#7,l.a=-110,l.dist=0.27w}{verta}
\fmfiv{label=#8,l.a=60,l.dist=0.01w}{vertb}
\fmfiv{label=#9,l.a=-60,l.dist=0.01w}{vertc}
%%% Workaround for MetaPost 1.504 bug 
\fmfcmd{pair fubara; fubara = vloc(__v1);} 
\fmfiv{decor.shape=circle,decor.filled=full,decor.size=3}{fubara}
\end{fmfchar*}}}}%}

\newcommand{\diaglttold}[6][]{%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-7.5\unitlength}%
%\smash[b]{%
\raisebox{\eqoff}{%
\fmfframe(1,0)(1,0){%
\begin{fmfchar*}(20,15)
\fmfleft{v1}
\fmfright{v0,v2,v5,v6,v7,v3,v4}
\fmf{#2,right=0.2,tension=0.6}{v1,vc1}
\fmf{#3,left=0.2,tension=0.6}{v1,vc2}
\fmf{#4,tension=0.1}{vc1,vc2}
\fmf{#5}{vc1,v2}
\fmf{#6}{vc2,v3}
\fmffreeze
\fmfposition
\fmfipath{p[]}
\fmfipair{vm[]}
\fmfiset{p1}{vpath(__v1,__vc1)}
\fmfiset{p2}{vpath(__vc1,__vc2)}
\fmfiset{p3}{reverse vpath(__vc2,__vc1) }
\fmfiset{p4}{vpath(__vc2,__v2)}
% \svertex{vm1}{p2}
% \svertex{vm2}{p3}
{#1}
%%% Workaround for MetaPost 1.504 bug 
\fmfcmd{pair fubara; fubara = vloc(__v1);} 
\fmfiv{decor.shape=circle,decor.filled=full,decor.size=3}{fubara}
\end{fmfchar*}}}}%}

\newcommand{\diagltx}[8]{%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-7.5\unitlength}%
%\smash[b]{%
\raisebox{\eqoff}{%
\fmfframe(0,0)(4,0){%
\begin{fmfchar*}(20,15)
\fmfleft{v1}
\fmfright{v0,v2,v5,v6,v7,v3,v4}
\fmf{#1,left=0.7,tension=1}{v1,vc1}
\fmf{#2,right=0.7,tension=1}{v1,vc1}
\fmf{#3,right=0.2}{vc1,v2}
\fmf{#4,left=0.2}{vc1,v3}
\fmffreeze
\fmfposition
\fmfipath{p[]}
\fmfipair{vm[]}
\fmfiset{p1}{vpath(__v1,__vc1)}
\fmfiset{p2}{vpath(__vc1,__vc2)}
% \fmfiset{p3}{reverse vpath(__vc2,__vc1) }
\fmfiset{p3}{vpath(__vc1,__vc2)}
\fmfiset{p4}{vpath(__vc2,__v2)}
% \svertex{vm1}{p2}
% \svertex{vm2}{p3}
%%% Workaround for MetaPost 1.504 bug 
\fmfcmd{pair verta, vertb, vertc; verta = vloc(__v1); vertb = vloc(__v3); vertc = vloc(__v2);}
\fmfiv{label=#5,l.a=110,l.dist=0.27w}{verta}
\fmfiv{label=#6,l.a=-110,l.dist=0.27w}{verta}
\fmfiv{label=#7,l.a=60,l.dist=0.01w}{vertb}
\fmfiv{label=#8,l.a=-60,l.dist=0.01w}{vertc}
%%% Workaround for MetaPost 1.504 bug 
\fmfcmd{pair fubara; fubara = vloc(__v1);} 
\fmfiv{decor.shape=circle,decor.filled=full,decor.size=3}{fubara}
\end{fmfchar*}}}}%}


\newcommand{\diagltxblob}[8]{%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-7.5\unitlength}%
%\smash[b]{%
\raisebox{\eqoff}{%
\fmfframe(0,0)(4,0){%
\begin{fmfchar*}(20,15)
\fmfleft{v1}
\fmfright{v0,v2,v5,v6,v7,v3,v4}
\fmf{#1,left=0.7,tension=1}{v1,vc1}
\fmf{#2,right=0.7,tension=1}{v1,vc1}
\fmf{#3,right=0.2}{vc1,v2}
\fmf{#4,left=0.2}{vc1,v3} 
\fmfv{decor.shape=circle,decor.filled=full,decor.size=20}{vc1}
\fmffreeze
\fmfposition
\fmfipath{p[]}
\fmfipair{vm[]}
\fmfiset{p1}{vpath(__v1,__vc1)}
\fmfiset{p2}{vpath(__vc1,__vc2)}
% \fmfiset{p3}{reverse vpath(__vc2,__vc1) }
\fmfiset{p3}{vpath(__vc1,__vc2)}
\fmfiset{p4}{vpath(__vc2,__v2)}
% \svertex{vm1}{p2}
% \svertex{vm2}{p3}
%%% Workaround for MetaPost 1.504 bug 
\fmfcmd{pair verta, vertb, vertc; verta = vloc(__v1); vertb = vloc(__v3); vertc = vloc(__v2);}
\fmfiv{label=#5,l.a=110,l.dist=0.27w}{verta}
\fmfiv{label=#6,l.a=-110,l.dist=0.27w}{verta}
\fmfiv{label=#7,l.a=60,l.dist=0.01w}{vertb}
\fmfiv{label=#8,l.a=-60,l.dist=0.01w}{vertc}
%%% Workaround for MetaPost 1.504 bug 
\fmfcmd{pair fubara; fubara = vloc(__v1);} 
\fmfiv{decor.shape=circle,decor.filled=full,decor.size=3}{fubara}
\end{fmfchar*}}}}%}


\newcommand{\diagltxold}[5][]{%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-7.5\unitlength}%
%\smash[b]{%
\raisebox{\eqoff}{%
\fmfframe(1,0)(1,0){%
\begin{fmfchar*}(20,15)
\fmfleft{v1}
\fmfright{v0,v2,v5,v6,v7,v3,v4}
\fmf{#2,left=0.7,tension=1}{v1,vc1}
\fmf{#3,right=0.7,tension=1}{v1,vc1}
\fmf{#4,right=0.2}{vc1,v2}
\fmf{#5,left=0.2}{vc1,v3}
\fmffreeze
\fmfposition
\fmfipath{p[]}
\fmfipair{vm[]}
\fmfiset{p1}{vpath(__v1,__vc1)}
\fmfiset{p2}{vpath(__vc1,__vc2)}
% \fmfiset{p3}{reverse vpath(__vc2,__vc1) }
\fmfiset{p3}{vpath(__vc1,__vc2)}
\fmfiset{p4}{vpath(__vc2,__v2)}
% \svertex{vm1}{p2}
% \svertex{vm2}{p3}
{#1}
%%% Workaround for MetaPost 1.504 bug 
\fmfcmd{pair fubara; fubara = vloc(__v1);} 
\fmfiv{decor.shape=circle,decor.filled=full,decor.size=3}{fubara}
\end{fmfchar*}}}}%}


\newcommand{\cvertr}[4][]{%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-9\unitlength}%
%\smash[b]{%
\raisebox{\eqoff}{%
\fmfframe(5,3)(5,3){%
\begin{fmfchar*}(12,12)
\fmfleft{v3,v1}
\fmfright{v2}
\fmf{#2}{v1,vc1}
\fmf{#3}{v2,vc1}
\fmf{#4}{v3,vc1}
\fmffreeze
\fmfposition
\fmfipath{p[]}
\fmfipair{vm[],vo[],vi[]}
\fmfiset{p1}{vpath(__v1,__vc1)}
\fmfiset{p2}{vpath(__v2,__vc1)}
\fmfiset{p3}{vpath(__v3,__vc1)}
% \svertex{vm1}{p1}
% \dvertex{vo1}{vi1}{p1}
% \svertex{vm2}{p2}
% \dvertex{vi2}{vo2}{p2}
% \svertex{vm3}{p3}
% \dvertex{vo3}{vi3}{p3}
{#1}
%\fmfiv{label=$\scriptstyle \alpha$,l.dist=2}{vloc(__v1)}
%\fmfiv{label=$\scriptstyle \beta$,l.dist=2}{vloc(__v2)}
%\fmfiv{label=$\scriptstyle \gamma$,l.dist=2}{vloc(__v3)}
\end{fmfchar*}}}%}
}

\newcommand{\qvertr}[5][]{%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-12\unitlength}%
%\smash[b]{%
\raisebox{\eqoff}{%
\fmfframe(4,6)(4,6){%
\begin{fmfchar*}(12,12)
\fmfleft{v1,v4}
\fmfright{v2,v3}
\fmfforce{(0,h)}{v1}
\fmfforce{(0,0)}{v4}
\fmfforce{(w,0)}{v3}
\fmfforce{(w,h)}{v2}
\fmf{#2}{v1,vc1}
\fmf{#3}{v2,vc1}
\fmf{#4}{v3,vc1}
\fmf{#5}{v4,vc1}
\fmffreeze
\fmfposition
\fmfipath{p[]}
\fmfipair{vm[],vo[],vi[]}
\fmfiset{p1}{vpath(__v1,__vc1)}
\fmfiset{p2}{vpath(__v2,__vc1)}
\fmfiset{p3}{vpath(__v3,__vc1)}
\fmfiset{p4}{vpath(__v4,__vc1)}
% \svertex{vm1}{p1}
% \dvertex{vo1}{vi1}{p1}
% \svertex{vm2}{p2}
% \dvertex{vi2}{vo2}{p2}
% \svertex{vm3}{p3}
% \svertex{vm4}{p4}
% \dvertex{vi4}{vo4}{p4}
{#1}
%\fmfiv{label=$\scriptstyle \alpha$,l.dist=2}{vloc(__v1)}
%\fmfiv{label=$\scriptstyle \beta$,l.dist=2}{vloc(__v2)}
%\fmfiv{label=$\scriptstyle \gamma$,l.dist=2}{vloc(__v3)}
\end{fmfchar*}}}%}
}


==> Macros/Macros.tex <==
%%%%% ABKÜRZUNGEN

%%% Math abbreviations

% sets
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\CC}{\ensuremath{\mathbb{C}}}
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\NN}{\ensuremath{\mathbb{N}}}

% groups and algebras
\newcommand{\G}{\ensuremath{G}\xspace}
\newcommand{\UN}{\ensuremath{U(N)}\xspace}
\newcommand{\SUN}{\ensuremath{SU(N)}\xspace}
\newcommand{\U}[1]{\ensuremath{U(#1)}\xspace}
\newcommand{\SU}[1]{\ensuremath{SU(#1)}\xspace}
\newcommand{\SO}[1]{\ensuremath{SO(#1)}\xspace}
\newcommand{\GLs}[2]{\ensuremath{GL(#1|#2)}\xspace}
\newcommand{\SUs}[2]{\ensuremath{SU(#1|#2)}\xspace}
\newcommand{\PSLs}[2]{\ensuremath{PSL(#1|#2)}\xspace}
\newcommand{\galgebra}{\ensuremath{\mathfrak{g}}\xspace}
\newcommand{\su}[1]{\ensuremath{\mathfrak{su}(#1)}\xspace}
\newcommand{\so}[1]{\ensuremath{\mathfrak{so}(#1)}\xspace}
\newcommand{\psutctsf}{\ensuremath{\mathfrak{psu}(2,2|4)}\xspace}

% Misc
\newcommand{\complexi}{i}
\newcommand{\superQ}{\mathfrak{Q}}
\newcommand{\superQd}{\dot{\superQ}}
% \newcommand{\Dzero}{{D_0}}
\newcommand{\EulerPhi}{\varphi}
\newcommand{\DilatationD}{D}
\newcommand{\methodd}{d}
\newcommand{\methodD}{\methodd}
\newcommand{\what}{\hat{w}}
\newcommand{\yhat}{\hat{y}}
% \newcommand{\g}[1]{{\gamma_{#1}}}
% \newcommand{\cg}[1]{{\cos{\gamma_{#1}}}}
\DeclareMathOperator{\idm}{\mathds{1}}
\newcommand{\diag}{\text{diag}}
\newcommand{\phase}[2]{\e^{\complexi \mathbf{q}_{#1}\times \mathbf{q}_{#2}}}
\newcommand{\halfphase}[2]{\e^{\complexi (\mathbf{q}_{#1}\times \mathbf{q}_{#2})/2}}
\newcommand{\negphase}[2]{\e^{-\complexi \mathbf{q}_{#1}\times \mathbf{q}_{#2}}}
\newcommand{\Doperator}{\mathfrak{D}}
\newcommand{\anomalousdim}{\gamma}

\newcommand{\AdS}{\text{AdS}}
\newcommand{\CFT}{\text{CFT}}


%%% Math 

% Misc

\newcommand{\indups}[1]{_{\mathrm{\scriptscriptstyle #1}}}
\newcommand{\gym}{g\indups{YM}}
\newcommand{\YM}{{\mathrm{\scriptscriptstyle YM}}}
%  
% \newcommand{\g}[1]{{\gamma_{#1}}}
% \newcommand{\cg}[1]{{\cos{\gamma_{#1}}}}
%\DeclareMathOperator{\premax}[1]{max}
\newcommand{\maxset}[1]{\max{\{#1\}}}
\newcommand{\minset}[1]{\min{\{#1\}}}
\DeclareMathOperator{\tr}{tr}
\newcommand{\Tr}{\tr}
\newcommand{\rtr}[1]{\tr_{#1}}
\newcommand{\singleE}[2]{\operatorname{E}_{#1,#2}}
\newcommand{\E}[4]{\operatorname{E}_{#1,#2}\otimes\operatorname{E}_{#3,#4}}
%\newcommand{\func}[2][red]{\textcolor{#1}{f(#2)}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\deltafct}[1]{\delta(#1)}

\DeclareMathOperator{\phaneq}{\phantom{{}=}}
\newcommand{\phaneqtimes}{\qquad \times}
\newcommand{\dzeroev}{{D_0}}
\newcommand{\colors}{s}
\newcommand{\colorshat}{\hat{s}}
\newcommand{\metric}{\ensuremath{\eta}}
\newcommand{\signature}{\zeta} %{\varsigma}
\newcommand{\e}{\operatorname{e}}
\newcommand{\cstar}{\ensuremath{\ast}}
\newcommand{\numberdot}[1]{#1}
\newcommand{\qqqquad}{\qquad\qquad\qquad\qquad}
\newcommand{\qqqqquad}{\qquad\qquad\qquad\qquad\qquad}
\newcommand{\qqqqqquad}{\qquad\qquad\qquad\qquad\qquad\qquad}

% brackets
\newcommand{\ev}[1]{\langle #1 \rangle}
\newcommand{\abs}[1]{|#1|}
\newcommand{\ket}[1]{\mid #1\,\rangle}
\newcommand{\nogapket}[1]{\mid \hspace{-0.2mm}\!#1\,\rangle}
\newcommand{\bra}[1]{\langle\,#1\,\mid}
\newcommand{\comm}[2]{[#1,#2]}
\newcommand{\acomm}[2]{\{#1,#2\}}
\newcommand{\starcomm}[2]{\comm{#1}{#2}_\cstar}
\newcommand{\staracomm}[2]{\acomm{#1}{#2}_\cstar}
\newcommand{\set}[1]{ \{ #1 \} }
\newcommand{\conditionset}[2]{\set{ #1 \operatorname{|} #2 }}
\newcommand{\state}[1]{\ket{#1}}
\newcommand{\vac}{\operatorname{\mid} 0 \, \operatorname{\rangle}}
\newcommand{\twositevac}{\state{0\,0}}


% equations
\newcommand{\eqndot}{\, .}
\newcommand{\eqncom}{\, ,}
\newcommand{\nn}{\nonumber}
\newcommand{\nnl}{\nonumber \\}


% Derivatives and integrals
\newcommand{\de}{\operatorname{d}\!}
\DeclareMathOperator{\dop}{d}
\newcommand{\measure}[1]{\dop\! #1}
\newcommand{\Diff}[2]{\frac{\dop^{#2}}{\dop\!{#1}^{#2}}}
\newcommand{\IntOp}[3]{\int^{#3}_{#2} \!\!\! \dop\! #1 \,}
\newcommand{\textIntOp}[3]{\int^{#3}_{#2} \! \dop\! #1 \,}
\newcommand{\MomInt}[2]{\int \frac{\dop^{#2}\!{#1}}{(2\pi)^{#2}}}

%%% References

\newcommand{\appref}[1]{appendix~\ref{#1}}
\newcommand{\Appref}[1]{Appendix~\ref{#1}}
\newcommand{\chapref}[1]{chapter~\ref{#1}}
\newcommand{\Chapref}[1]{Chapter~\ref{#1}}
\newcommand{\secref}[1]{section~\ref{#1}}
\newcommand{\Secref}[1]{Section~\ref{#1}}
\newcommand{\subsecref}[1]{subsection~\ref{#1}}
\newcommand{\tabref}[1]{table~\ref{#1}}
\newcommand{\figref}[1]{figure~\ref{#1}}

%%% Letters

% cal
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

% bold
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bq}{\mathbf{q}}

% dotted
\newcommand{\alphadot}{\dot{\alpha}}
\newcommand{\betadot}{\dot{\beta}}
\newcommand{\gammadot}{\dot{\gamma}}
\newcommand{\deltadot}{\dot{\delta}}
\newcommand{\epsilondot}{\dot{\epsilon}}


%%% Text abbreviations
\newcommand{\thooft}{'t~Hooft\xspace} 
% \renewcommand{\TH}{\ensuremath{T_{\text{H}}}}
\newcommand{\THag}{\ensuremath{T_{\text{H}}}}
\renewcommand{\H}{{\text{H}}}
\newcommand{\QCD}{{\text{QCD}}}
\newcommand{\stringc}{{\text{s}}}
\newcommand{\AdSCFT}{AdS/CFT\xspace}
\newcommand{\AdSCFTc}{AdS/CFT correspondence\xspace}
\newcommand{\Polya}{P\'{o}lya\xspace}
\newcommand{\Poincare}{Poincar\'{e}\xspace}
\newcommand{\RxSt}{\ensuremath{\mathbb{R}\times S^3}\xspace}
\newcommand{\Nfour}{$\mathcal{N}=4$\xspace}
\newcommand{\NfSYM}{\Nfour SYM\xspace}
\newcommand{\NfSYMt}{\Nfour SYM theory\xspace}
\newcommand{\AdS}[1]{\ensuremath{AdS_{#1}}\xspace}
\newcommand{\gidef}{${\gamma}_{i}$-deformation\xspace}
\newcommand{\gidefd}{${\gamma}_{i}$-de\-formed\xspace}
\newcommand{\expectationvalue}{expectation value\xspace}
\newcommand{\expectationvalues}{expectation values\xspace}

% Fields
\newcommand{\ferm}{\psi}
\newcommand{\antiferm}{\bar{\psi}}
\newcommand{\apferm}{\ferm}
\newcommand{\apantiferm}{\antiferm}
\newcommand{\sufphi}{\varphi}
\newcommand{\cfstrength}{\cF}
\newcommand{\cantifstrength}{\bar{\cfstrength}}
\newcommand{\fstrength}{F}
\newcommand{\antifstrength}{\bar{\fstrength}}
\newcommand{\gaugefield}{A}
\newcommand{\fieldstrength}{\fstrength}
\newcommand{\cder}{D}

% Oscillators
\newcommand{\aosc}{\ba}
\newcommand{\aoscdag}{\aosc^\dagger}
\newcommand{\bosc}{\bb}
\newcommand{\boscdag}{\bosc^\dagger}
\newcommand{\cosc}{\bc}
\newcommand{\coscdag}{\cosc^\dagger}

% occupation numbers
\newcommand{\akind}[1][ ]{a^{#1}}
\newcommand{\bkind}[1][ ]{b^{#1}}
\newcommand{\ckind}[1][ ]{c^{#1}}
\newcommand{\dkind}[1][ ]{d^{#1}}
\newcommand{\akindsite}[2][ ]{a^{#1}_{(#2)}}
\newcommand{\bkindsite}[2][ ]{b^{#1}_{(#2)}}
\newcommand{\ckindsite}[2][ ]{c^{#1}_{(#2)}}
\newcommand{\dkindsite}[2][ ]{d^{#1}_{(#2)}}
\newcommand{\nsite}[1]{n_{(#1)}}

% operators
\newcommand{\centralchargeop}{\ensuremath{\mathcal{C}}}
\newcommand{\centralchargeopdensity}{\ensuremath{C}}
\newcommand{\centralchargeoperatordensity}{\centralchargeopdensity}
\newcommand{\oneloopdop}{\ensuremath{\mathfrak{D}_2}}
\newcommand{\Dzerodensity}{\ensuremath{D_0}}
\newcommand{\Dtwodensity}{\ensuremath{D_2}}
\newcommand{\Dzero}{\ensuremath{\mathfrak{D}_0}}
\newcommand{\Dtwo}{\ensuremath{\mathfrak{D}_2}}


% algebra generators
\newcommand{\Drealalg}{\ensuremath{\mathscr{D}}}
\newcommand{\Prealalg}{\ensuremath{\mathscr{P}}}
\newcommand{\Krealalg}{\ensuremath{\mathscr{K}}}
\newcommand{\Lrealalg}{\ensuremath{\mathscr{L}}}
\newcommand{\Jrealalg}{\ensuremath{\mathscr{J}}}


% Operators
\newcommand{\Dalg}{\ensuremath{\mathfrak{D}}}
\newcommand{\Halg}{\ensuremath{\mathfrak{H}}}


% Colour
\DeclareMathOperator{\T}{T}
\newcommand{\onetrace}[1]{\tr\T^{#1}}
\newcommand{\twotrace}[2]{\tr\T^{#1}\T^{#2}}
\newcommand{\threetrace}[3]{\tr\T^{#1}\T^{#2}\T^{#3}}
\newcommand{\fourtrace}[4]{\tr\T^{#1}\T^{#2}\T^{#3}\T^{#4}}
\newcommand{\threetracecomm}[3]{\tr\T^{#1}\comm{\T^{#2}}{\T^{#3}}}

% Coupling tensors

\newcommand{\Qtilde}[4]{\tilde{Q}_{#4 #3}^{#1 #2}}
\newcommand{\Qbare}[4]{Q_{ #4 #3}^{#1 #2}}
\newcommand{\Qhat}[4]{\hat{Q}_{#4 #3}^{#1 #2}}

\newcommand{\Qt}[4]{\Qtilde{#1}{#2}{#3}{#4}}
\newcommand{\Qonehalf}[4]{\Qbare{#1}{#2}{#3}{#4}}
\newcommand{\Q}[4]{\Qhat{#1}{#2}{#3}{#4}}

\newcommand{\ro}[3]{({\rho}_{#1})_{#2 #3}}
\newcommand{\rodag}[3]{(\rho^{\dagger #1})^{#2 #3}}
\newcommand{\rotil}[3]{(\tilde{\rho}_{#1})^{#2 #3}}
\newcommand{\rotildag}[3]{(\tilde{\rho}^{\dagger #1})_{#2 #3}}


% Christoph stuff
\newlength{\eqoff}

% SUSY stuff
\DeclareMathOperator{\D}{D}
\DeclareMathOperator{\barD}{\vphantom{\D}\smash[t]{\bar{\mathrm{D}}}}



